Time-Optimal Sublinear Algorithms for Matching and Vertex Cover

We study the problem of estimating the size of maximum matching and minimum vertex cover in sublinear time. Denoting the number of vertices by $n$ and the average degree in the graph by $\bar{d}$, we obtain the following results for both problems: * A multiplicative $(2+\epsilon)$-approximation that takes $\tilde{O}(n/\epsilon^2)$ time using adjacency list queries. * A multiplicative-additive $(2, \epsilon n)$-approximation in $\tilde{O}((\bar{d} + 1)/\epsilon^2)$ time using adjacency list queries. * A multiplicative-additive $(2, \epsilon n)$-approximation in $\tilde{O}(n/\epsilon^{3})$ time using adjacency matrix queries. All three results are provably time-optimal up to polylogarithmic factors culminating a long line of work on these problems. Our main contribution and the key ingredient leading to the bounds above is a new and near-tight analysis of the average query complexity of the randomized greedy maximal matching algorithm which improves upon a seminal result of Yoshida, Yamamoto, and Ito [STOC'09].

==> open.tex <==
In this paper, we gave a near-tight analysis of the average query-complexity of the randomized greedy maximal matching algorithm (Theorem~\ref{thm:querycomplexity}). This leads to several sublinear time algorithms (Theorems~\ref{thm:adjlist-multiplicative}, \ref{thm:adjlist-additive}, and \ref{thm:adjmatrix}) for estimating the size of maximum matching and minimum vertex cover in both the adjacency list query model and the adjacency matrix query model. 

While all of our algorithms have matching time-complexity lower bounds as discussed in Section~\ref{sec:intro}, it would be interesting to see if one can improve the approximation ratio of our algorithms. Particularly, does there exist a $(2-\epsilon_0)$-approximate estimator for maximum matching in the adjacency list model that makes $o(n^2)$ queries for all graphs? How about a $(2-\epsilon_0, \epsilon n)$ solution?


